Multiple Star Systems in the Orion Nebula

This work presents an interferometric study of the massive-binary fraction in the Orion Trapezium Cluster with the recently comissioned GRAVITY instrument. We observe a total of 16 stars of mainly OB spectral type. We find three previously unknown companions for $\theta ^1$ Ori B, $\theta ^2$ Ori B, and $\theta ^2$ Ori C. We determine a separation for the previously suspected companion of NU Ori. We confirm four companions for $\theta ^1$ Ori A, $\theta ^1$ Ori C, $\theta ^1$ Ori D, and $\theta ^2$ Ori A, all with substantially improved astrometry and photometric mass estimates. We refine the orbit of the eccentric high-mass binary $\theta ^1$ Ori C and we are able to derive a new orbit for $\theta ^1$ Ori D. We find a system mass of 21.7 $M_{\odot}$ and a period of $53$ days. Together with other previously detected companions seen in spectroscopy or direct imaging, eleven of the 16 high-mass stars are multiple systems. We obtain a total number of 22 companions with separations up to 600 AU. The companion fraction of the early B and O stars in our sample is about 2, significantly higher than in earlier studies of mostly OB associations. The separation distribution hints towards a bimodality. Such a bimodality has been previously found in A stars, but rarely in OB binaries, which up to this point have been assumed to be mostly compact with a tail of wider companions. We also do not find a substantial population of equal-mass binaries. The observed distribution of mass ratios declines steeply with mass, and like the direct star counts, indicates that our companions follow a standard power law initial mass function. Again, this is in contrast to earlier findings of flat mass ratio distributions in OB associations. We exclude collision as a dominant formation mechanism but find no clear preference for core accretion or competitive accretion.

==> include/dataanalysis.tex <==
\chapter{Data analysis}\label{chap:DataAnalysis}
%binary model fit, additional fits with candid and litpro for comparison
%The position fit of the binary was done in three separate ways to avoid fitting errors and false companions. The results of the three methods where compared for each observation and evaluated according to their accuracy. 
%
%\subsubsection{CANDID}
%
%The binary position was fitted with CANDID version (....) (verweis auf papaer), using the fitMap function and the bootstrapping method. 
%
%
%\subsubsection{Litpro}
%
%Another binary position fit was done with Litpro (...)
%
%\subsubsection{own Fit}

%As a third method, a t
\section{Modeling a binary star}\label{sec:binary model}

\subsection{Modeling the visibility}\label{ssec:vilibility_model}
Visibility of a binary model is described as

\begin{equation}\label{eq:binary_model}
\nu _{bin} = \dfrac{ \nu _{main} + f \cdot \nu _{comp}  \exp \left( -2i  \pi \dfrac{ u \cdot \Delta \alpha + v \cdot \Delta \delta }{ \lambda} \right) } {\left( 1 + f \right) },
\end{equation} %TODO reference!!
where $\nu_{main}$ and $\nu_{comp}$ are the complex visibilities for the main and the companion star, respectively. In most cases the star is unresolved, thus $\nu_{main} = \nu_{comp} = 1$. The parameters $u$, $v$ are the spatial frequencies of the telescope baselines, $\lambda$ is the observed wavelength, $\Delta \alpha $ and $\Delta \delta$ are the angular distances of the companion star from the primary star in RA and DEC, respectively, and $f = f_{comp}/f_{main}$ is the mean flux ratio over all wavelengths of the system, where $f_{comp}$ and $f_{main}$ are the flux of the companion star and primary star, respectively. 

The parameters $u, v ~\text{and}~ \lambda$ are provided by the observational data, while the distances $\Delta \alpha$ and $\Delta \delta$ together with the flux ratio $f$ are variable parameters to be fitted. To find starting values for these parameters, we use a grid-search algorithm, where we scan $\Delta \alpha$ and $\Delta \delta$ between either $\pm$200~mas, $\pm$100~mas or $\pm$50~mas in steps of either 1 or 0.5~mas, and the flux ratio $f$ between 0 and 1 in steps of 0.1. The best result of the grid-search forms the starting values for the subsequent weighted least-squares optimization (eq. \ref{eq:chi2}), using the Levenberg-Marquardt algorithm and the LMFIT package \citep{newville_2014_11813}.

\begin{equation}\label{eq:chi2}
\chi ^2 =\sum\limits_{i} \left( \dfrac{\nu_{Data,i} - \nu_{Model,i}}{error_{Data,i}} \right) ^2
\end{equation}

An example for the observed visibility and the optimized model visibility is shown in Figure \ref{fig:vis_fit_example}. The data were taken at the 20th March 2017, the observed object was $\theta ^1$ Ori B.

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{"../../theta1_Ori_B1_2017-03-20T00:36:33_v2"}
\caption{Observed visibilities and the fitted model visibility for the observation of $\theta ^1$ Ori B at the 20th March 2017.}\label{fig:vis_fit_example}
\end{figure}

\subsection{Modeling the closure phase and triple amplitude}
The closure phase is computed by taking the argument of the bispectrum (see subsection \ref{ssec:CPandT3}). The bispectrum is the product of complex visibilites for telescopes $i,j,k$:
\begin{equation} 
CP(i,j,k) = \arg \left( \nu_{bin,ij} \nu_{bin,jk} \nu_{bin,ki} \right)
\end{equation}
where the complex visibilites $\nu_{bin}$ are computed using eq. \ref{eq:binary_model}.

The triple amplitude is the modulus of the bispectrum. As expained in subsection \ref{ssec:CPandT3}, the most information is in the closure phase. Thus, the triple amplitude is not always necessary for fitting the data. 

The optimization is done in the same way as described in the previous subsection \ref{ssec:vilibility_model}. An example of the closure phase, triple amplitude and the resulting fitted model is shown in Figure \ref{fig:cp_t3_fit_example}. The data were taken at the 20th March 2017 of $\theta ^1$ Ori B. 

\begin{figure}
\begin{minipage}{0.5\textwidth}
\includegraphics[width=\textwidth]{"../../theta1_Ori_B1_2017-03-20T00:36:33_icp"}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\includegraphics[width=\textwidth]{"../../theta1_Ori_B1_2017-03-20T00:36:33_t3"}
\end{minipage}
\caption{Left: observed closure phase and model fit. Right: observed triple amplitude and the optimized model function. Data were taken at the 20th March 2017 of $\theta ^1$ Ori B.}\label{fig:cp_t3_fit_example}
\end{figure}

\section{Orbit modeling}

For fitting the orbit, we use the KeplerEllipse class of PyAstronomy\footnote{https://github.com/sczesla/PyAstronomy} to determine the position at a given time. This position is then compared with the obtained positions from the binary model fit (see section \ref{sec:binary model}) using equation \ref{eq:chi2}. The optimization is done with the Trust-region method, which supports boundaries of variables.

The parameters of the orbit are defined as following (see also Figure \ref{fig:orbital_elements}): $a$ is the major half axis of the Kepler ellipse, $P$ is the orbital period, $e$ the eccentricity, $\tau$ the time of periapsis passage, $\Omega$ the longitude of the ascending node, $\omega$ the argument of periapsis and $i$ the inclination of the orbit. The ascending node is defined as the point where the orbiting object passes the plan of reference in the direction of the observer. For a more detailed discussion see \citep[pp. 22-24]{2005ormo.book.....R}.

As an observer, we see the 3D-Orbit projected on a 2D-plane (plane of reference in figure \ref{fig:orbital_elements}).  The projection of different orbits can appear similar on the plane of reference, e.g. a highly inclined and eccentric orbit can appear as a not inclined circular orbit. In order to not get stuck in a local minimum of $\chi ^2$, a good starting value is essential for optimization. If orbital elements are already determined in the literature, we take these elements as starting value for the optimization, e.g the values from \citet{Kraus2009} for the orbit of $\theta ^1$ Ori C$_2$ (see subsection \ref{ssec:t1C}). If there are no previously determined orbital elements, we use the Basin-Hopping algorithm \citep{Wales1997}, to find a global minimum and use the result as starting value for the Trust-region method.


\begin{figure}
\centering
\tdplotsetmaincoords{70}{110}
\begin{tikzpicture}[tdplot_main_coords,scale=5]
  \pgfmathsetmacro{\r}{.8}
  \pgfmathsetmacro{\O}{45} % right ascension of ascending node [deg]
  \pgfmathsetmacro{\i}{30} % inclination [deg]
  \pgfmathsetmacro{\f}{35} % true anomaly [deg]




  \coordinate (O) at (0,0,0);


 % \draw [->] (O) -- (2,0,0) node[anchor=north east] {$x$};
  %\draw [->] (O) -- (0,1,0) node[anchor=north west] {$y$};
  %\draw [->] (O) -- (0,0,1) node[anchor=south] {$z$};

  \tdplotdrawarc[dashed, fill=WhiteSmoke]{(O)}{\r}{225}{45}{anchor=south west}{Plane of reference}
 

  \tdplotsetrotatedcoords{\O}{0}{0}

  \draw [tdplot_rotated_coords] (-1,0,0) -- (1,0,0) node [below right] {Ascending node};
  \tdplotdrawarc[->]{(O)}{.33*\r}{0}{\O}{anchor=north}{$\Omega$}

  \tdplotsetrotatedcoords{-\O}{\i}{0}
  \tdplotdrawarc[tdplot_rotated_coords]{(O)}{\r}{0}{360}{}{}  
  \begin{scope}[tdplot_rotated_coords]

%    \draw[->] (O) -- (0,0,1) node [above] {$\hat{h}$};
    \draw (1,0,0) -- (-1,0,0);
    \tdplotdrawarc[thick, ->,color=deep2]{(O)}{.33*\r}{90}{180}{anchor=west}{$\omega$}
    \coordinate (P) at (180+\f:\r);
    \draw (O) -- (P);
  %  \tdplotdrawarc[->]{(O)}{.33*\r}{180}{180+\f}{anchor=south west}{$\nu$}
  \end{scope}

    \coordinate (I) at (45+0:\r);
  \tdplotsetrotatedcoords{-\O+\f}{\i}{0}
  \tdplotsetrotatedcoordsorigin{(P)}
  \begin{scope}[tdplot_rotated_coords,scale=.2,thick]
    \fill (P) circle (.33ex);
  \end{scope}



  
    \tdplotdrawarc[dashed, fill=WhiteSmoke]{(O)}{-\r}{225}{45}{}{}
    \coordinate (V) at (80+0:-\r-0.1);
    \draw [->] (O) -- (V) node[anchor=south] {\vernal};
      \node at (-0.2,-\r-0.15,-0.0) [left,text width=4em] {Point of reference};

    \tdplotdrawarc[thick, ->,color=deep1]{(O)}{-\r*0.5}{80}{225}{anchor=north east}{$\Omega$}
	\tdplotsetrotatedthetaplanecoords{90}
     \tdplotdrawarc[thick, tdplot_rotated_coords,->]{(I)}{0.5}{0}{\i}{anchor=south}{$i$}
\end{tikzpicture}
\caption{The orbital elements of a Kepler orbit. The plane of reference is in the observers field of view.}\label{fig:orbital_elements}
\end{figure}

\section{Dust extinction}
For calculating the Luminosity or absolute Magnitude of a star, we need to consider extinction effects of the interstellar medium. $A(\lambda)$ is the extinction at wavelength $\lambda$ in magnitudes. The extinction of color is described by $E(B-V) = A(B) - A(V)$. The interstellar reddening law is $R_V = A(V) / E(B-V)$. For the diffuse interstellar medium, a typical value is $R_V = 3.1$, whereas for dense clouds the value is $R_V = 5$ \citep[p. 527]{allen2000allen}. In the K-band and for $R_V = 3.1$ we get $A_V/E(V-K) = 1.13 \pm 0.003$ and thus $A_K = (0.115 \pm 0.003)  A_V$  \citep[p. 158]{allen2000allen}. 

\section{Detection Limits}\label{sec:candid}


